Planning Like Human: A Dual-process Framework for Dialogue Planning

In proactive dialogue, the challenge lies not just in generating responses but in steering conversations toward predetermined goals, a task where Large Language Models (LLMs) typically struggle due to their reactive nature. Traditional approaches to enhance dialogue planning in LLMs, ranging from elaborate prompt engineering to the integration of policy networks, either face efficiency issues or deliver suboptimal performance. Inspired by the dualprocess theory in psychology, which identifies two distinct modes of thinking - intuitive (fast) and analytical (slow), we propose the Dual-Process Dialogue Planning (DPDP) framework. DPDP embodies this theory through two complementary planning systems: an instinctive policy model for familiar contexts and a deliberative Monte Carlo Tree Search (MCTS) mechanism for complex, novel scenarios. This dual strategy is further coupled with a novel two-stage training regimen: offline Reinforcement Learning for robust initial policy model formation followed by MCTS-enhanced on-the-fly learning, which ensures a dynamic balance between efficiency and strategic depth. Our empirical evaluations across diverse dialogue tasks affirm DPDP's superiority in achieving both high-quality dialogues and operational efficiency, outpacing existing methods.

==> Algorithms/algorithm_1.tex <==
\begin{algorithm}[!h]
    \caption{Algorithm of SUM}
    \label{alg:AOS}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    
    \begin{algorithmic}[1]
        \REQUIRE $A$, $B$, $C$(This is Inputs)  %%input
        \ENSURE XXX(This is Outputs)    %%output
        
        \STATE  xxxxx
        
        \WHILE{$A=B$}
            \STATE xxxxx
        \ENDWHILE
        
        \FOR{each $i \in [1,10]$}
            \IF {$C = 0$}
                \STATE xxxxx
            \ELSE
                \STATE xxxxx
            \ENDIF
        \ENDFOR
        
        \RETURN Outputs
    \end{algorithmic}
\end{algorithm}

==> Algorithms/algorithm_2.tex <==
\begin{algorithm}[!h]
    \caption{MCTS-guided Policy Training}
    \label{alg:AOS}
    \renewcommand{\algorithmicrequire}{\textbf{Require:}}
    \renewcommand{\algorithmicensure}{\textbf{Ensure:}}
    
    \begin{algorithmic}[1]
        \REQUIRE $LLM$  %%input
        \ENSURE XXX(This is Outputs)    %%output
        
        \STATE  xxxxx
        
        \WHILE{$A=B$}
            \STATE xxxxx
        \ENDWHILE
        
        \FOR{each $i \in [1,10]$}
            \IF {$C = 0$}
                \STATE xxxxx
            \ELSE
                \STATE xxxxx
            \ENDIF
        \ENDFOR
        
        \RETURN Outputs
    \end{algorithmic}
\end{algorithm}

==> Sections/abstract_0.tex <==
\begin{abstract}
% Effective dialogue planning plays a significant role in addressing the challenges of proactive dialogue. Although existing prompting approaches with large language models (LLMs) present fair performance, their limitations become apparent within the constraints of frozen LLM. PPDPP overcomes this by learning a small neural policy agent to guide LLMs' responses. However, the planning mechanism of PPDPP primarily focuses on predicting actions based on current dialogue histories, overlooking simulating possible future states to assist current decisions.
% % Drawing inspiration from the dual-process theory, we divide the dialogue responses into intuitive ones under familiar situations and thoughtful ones under unfamiliar scenarios. 
% According to existing dual-process theory, human dialogue responses can be divided into intuitive actions that respond quickly without considering subsequent influences, and thoughtful behaviors by simulating subsequent dialogue rounds and possible impacts.
% Motivated by this theory, we introduce a dual-process dialogue planning framework, just like humans do. Specifically, we employ a policy network and Monte Carlo Tree Search (MCTS) to emulate these two cognitive processes and seamlessly integrate them using a parameterless control mechanism.
% To enhance the dialogue planning abilities of the policy network under the intuitive process, we propose a two-stage training approach involving Offline Reinforcement Learning-based pretraining and MCTS-guided self-play training.
% Our approach significantly outperforms PPDPP on two datasets, highlighting the advantages of our proposed dual-process planning framework and two-stage policy training method.
% Effective dialogue planning is crucial for addressing the challenges inherent in proactive dialogue. Existing prompting methods using large language models (LLMs) show decent performance, but their effectiveness is limited by the static nature of LLMs. Subsequent studies overcome this by employing a small neural policy network to steer LLM responses.
% However, the planning mechanism of this neural policy network mainly predicts actions based on current dialogue histories and neglects simulating future states to assist current decision-making.
% According to the established dual-process theory, human dialogue responses entail both intuitive actions being swiftly executed without considering subsequent influences, and thoughtful behaviors that consider subsequent dialogue rounds and their potential impacts.
% Motivated by this theory, we propose a dual-process dialogue planning framework mirroring human cognitive processes. Specifically, we employ a policy network and Monte Carlo Tree Search (MCTS) to emulate these two cognitive processes, seamlessly integrating them through a parameterless control mechanism. To enhance the dialogue planning capabilities of intuitive planning, we advocate a two-stage training regimen encompassing Offline Reinforcement Learning-based pretraining followed by MCTS-guided self-play training.
% Our proposed approach markedly outperforms a series of baselines across two datasets, underscoring the superiority of our dual-process planning framework and two-stage policy training method.
Effective dialogue planning is essential for tackling the challenges inherent in proactive dialogue. Current prompting methods employing large language models (LLMs) exhibit mediocre performance since being hindered by the frozen nature of LLMs. Subsequent studies have addressed this by employing a small neural policy network to guide LLM responses. However, the planning mechanism of this neural policy network primarily predicts actions based on current dialogue histories, neglecting to think of future reactions to aid in current decision-making. 
According to the established dual-process theory, human dialogue responses encompass both intuitive actions swiftly executed without considering subsequent influences, and thoughtful behaviors considering possible impacts of subsequent dialogue rounds. Motivated by this theory, we propose a dual-process dialogue planning framework that mirrors human cognitive processes. 
To enhance the dialogue planning capabilities of the framework, we propose a two-stage training regimen comprising Offline Reinforcement Learning-based pretraining followed by MCTS-guided self-play training. Our proposed approach significantly outperforms several baselines across two datasets, highlighting the superiority of our dual-process planning framework and two-stage policy training method.

\end{abstract}

==> Sections/acknowledgements.tex <==
\section*{Acknowledgements}

==> Tables/cb_results.tex <==
\begin{table}[t]
    \centering
    \renewcommand*{\arraystretch}{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{CraisglistBargain}}\\
    & AT$\downarrow$ & SR$\uparrow$ & SL$\uparrow$\\
    \midrule
    \multicolumn{1}{l}{DialoGPT~\cite{zhang2019dialogpt}} & 6.73 & 0.3245 & 0.2012 \\
    \midrule
    \multicolumn{1}{l}{Standard} & 6.47 & 0.3830 & 0.1588 \\
    \multicolumn{1}{l}{AnE~\cite{zhang2023ask}} & 5.91 & 0.4521 & 0.2608 \\
    \multicolumn{1}{l}{Proactive~\cite{deng2023prompting}} & 5.80 & 0.5638 & 0.2489 \\
    \multicolumn{1}{l}{ProCoT~\cite{deng2023prompting}} & 6.22 & 0.5319 & 0.2486 \\
    \multicolumn{1}{l}{ICL-AIF~\cite{fu2023improving}} & 6.53 & 0.3617 & 0.1881 \\
    \multicolumn{1}{l}{PPDPP~\cite{deng2023plug}} & 5.62 & 0.6117 & \underline{0.3376} \\
    \multicolumn{1}{l}{$\quad$-w/o SFT} & 5.71 & 0.6223 & 0.3354 \\
    \multicolumn{1}{l}{$\quad$-w/o RL} & \underline{5.57} & \underline{0.6649} & 0.2280 \\
    \midrule
    \midrule
    \multicolumn{1}{l}{DPDP (System 1)} & {5.03} & {0.7447} & \textbf{0.4108}  \\
    \multicolumn{1}{l}{{DPDP (System 1\&2, 22.3\% MCTS)}} & {3.69} & {0.8298} & {0.3102} \\
    \multicolumn{1}{l}{{DPDP (System 1\&2, 51.4\% MCTS)}} & {2.77} & {0.9468} & {0.3118} \\
    \multicolumn{1}{l}{{DPDP (System 1\&2, 60.3\% MCTS)}} & \textbf{2.49} & {0.9681} & {0.2856} \\
    \multicolumn{1}{l}{{DPDP (System 2)}} & 2.78 & \textbf{0.9734} & 0.2728 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Experimental results on CraisglistBargain. PT means Pretraining and SPT means Self-Play Training.}
    \label{tab:cb_results}
\end{table}

==> Tables/datasets.tex <==
\begin{table}[!t]
    \centering
    \caption{The statistics of datasets.}
    \begin{tabular}{lrrrrr}
    \toprule
    Dataset& \# Case & \# Action \\
    \midrule
    ESConv & 1040/130/130 & 8 \\
    CIMA & 909/113/113 & 5 \\
    \bottomrule
    \end{tabular}
    \label{tab:dataset_statistics}
\end{table}

==> Tables/human_eval.tex <==
% \begin{table}[!t]
%     \centering
%     \caption{Human evaluation results.}
%     \subtable[ESConv]{
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccccccc}
%     \toprule
%     DPDP (Policy) & \multicolumn{2}{c}{Ide.} & \multicolumn{2}{c}{Com.} & \multicolumn{2}{c}{Sug.} & \multicolumn{2}{c}{Com.} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
%     vs. & Win & Lose & Win & Lose & Win & Lose & Win & Lose \\
%     \midrule
%     PPDPP &  &  &  &  &  &  &  &  \\
%     \bottomrule
%     \end{tabular}
%     }
%     }
%     \subtable[CIMA]{
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccccccc}
%     \toprule
%     DPDP (Policy) & \multicolumn{2}{c}{Hint} & \multicolumn{2}{c}{Identity} & \multicolumn{2}{c}{Correct} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
%     vs. & Win & Lose & Win & Lose & Win & Lose \\
%     \midrule
%     PPDPP &  &  &  &  &  &  \\
%     \bottomrule
%     \end{tabular}
%     }
%     }
%     \label{tab:human_eval}
% \end{table}


\begin{table}[!t]
    \centering
    \caption{Human evaluation results on ESConv.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
    DPDP (System 1) & \multicolumn{2}{c}{Sug.} & \multicolumn{2}{c}{Com.} & \multicolumn{2}{c}{Ide.} & \multicolumn{2}{c}{Ove.} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
    vs. & Win & Lose & Win & Lose & Win & Lose & Win & Lose \\
    \midrule
    PPDPP & 59\% & 15\% & 26\% & 46\% & 29\% & 31\% & 59\% & 24\% \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:human_eval}
\end{table}

==> Tables/trade_off_mcts_ratio.tex <==
\begin{table}[!t]
    \centering
    \caption{SR and AT results of employing different proportions of MCTS on ESConv and CIMA.}
    \subtable[ESConv]{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    & \textbf{0.0\%} & \textbf{21.9\%} & \textbf{46.5\%} & \textbf{68.3\%} & \textbf{100.0\%} \\
    \midrule
    \textbf{SR} & 0.9000 & 0.9154 & 0.9692 & 0.9769 & 0.9923 \\
    \textbf{AT} & 3.61 & 3.42 & 2.95 & 2.72 & 2.13 \\
    \bottomrule
    \end{tabular}
    }
    }
    \subtable[CIMA]{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    & \textbf{0.0\%} & \textbf{28.6\%} & \textbf{50.0\%} & \textbf{81.1\%} & \textbf{100.0\%} \\
    \midrule
    \textbf{SR} & 0.9469 & 0.9646 & 0.9823 & 0.9735 & 0.9735 \\
    \textbf{AT} & 2.24 & 2.39 & 2.28 & 2.58 & 2.49 \\
    \bottomrule
    \end{tabular}
    }
    }
    \label{tab:trade_off_mcts}
\end{table}


% \begin{table}[t]
%     \centering
%     \caption{Experimental results on ESConv and CIMA. PT means Pretraining and SPT means Self-Play Training.}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lcclcc}
%     \toprule
%     \multirow{2}{*}{\textbf{Ratios (\%)}} & \multicolumn{2}{c}{\textbf{ESConv}} & \multirow{2}{*}{\textbf{Ratios}} & \multicolumn{2}{c}{\textbf{CIMA}}\\
%     & AT$\downarrow$ & SR$\uparrow$ & AT$\downarrow$ & SR$\uparrow$\\
%     \midrule
%     \multicolumn{1}{l}{0.0} & 5.31 & 0.7538 & 5.43 & 0.4956 \\
%     \midrule
%     \multicolumn{1}{l}{21.9} & 5.10 & 0.7692 & 3.89 & 0.6903 \\
%     \multicolumn{1}{l}{AnE~\cite{zhang2023ask}} & 4.76 & 0.8000 & 3.86 & 0.6549 \\
%     \multicolumn{1}{l}{Proactive~\cite{deng2023prompting}} & 5.08 & 0.7538 & 4.84 & 0.5310 \\
%     \multicolumn{1}{l}{ProCoT~\cite{deng2023prompting}} & 4.75 & 0.7923 & 4.58 & 0.5487 \\
%     \multicolumn{1}{l}{ICL-AIF~\cite{fu2023improving}} & 4.69 & 0.8079 & 4.19 & 0.6106 \\
%     \multicolumn{1}{l}{PPDPP~\cite{deng2023plug}} & \underline{4.56} & \underline{0.8462} & \underline{3.03} & \underline{0.8407} \\
%     \midrule
%     \midrule
%     \multicolumn{1}{l}{DPDP (System 1)} & {3.61} & {0.9000} & \textbf{2.24} & {0.9469} \\
%     \multicolumn{1}{l}{$\quad$-w/o PT} & 4.22 & 0.8769 & 2.36 & 0.9292 \\
%     \multicolumn{1}{l}{$\quad$-w/o SPT} & 3.97 & 0.8692 & 2.51 & 0.8938 \\
%     \multicolumn{1}{l}{{DPDP (System 2)}} & {2.13} & {0.9923} & {2.49} & {0.9735} \\
%     \multicolumn{1}{l}{{DPDP (System 1\&2)}} & \textbf{2.13} & \textbf{0.9923} & {2.28} & \textbf{0.9823} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:static_results}
% \end{table}
